Two Computational Models for Analyzing Political Attention in Social Media

Understanding how political attention is divided and over what subjects is crucial for research on areas such as agenda setting, framing, and political rhetoric. Existing methods for measuring attention, such as manual labeling according to established codebooks, are expensive and can be restrictive. We describe two computational models that automatically distinguish topics in politicians' social media content. Our models---one supervised classifier and one unsupervised topic model---provide different benefits. The supervised classifier reduces the labor required to classify content according to pre-determined topic list. However, tweets do more than communicate policy positions. Our unsupervised model uncovers both political topics and other Twitter uses (e.g., constituent service). These models are effective, inexpensive computational tools for political communication and social media research. We demonstrate their utility and discuss the different analyses they afford by applying both models to the tweets posted by members of the 115th U.S. Congress.

==> revision-table.tex <==
% \usepackage[math]{cellspace}
% \cellspacetoplimit 4pt
% \cellspacebottomlimit 4pt
\pagenumbering{gobble}

\newcolumntype{A}{>{\raggedright\arraybackslash}m{6cm}}
\newcolumntype{B}{>{\raggedright\arraybackslash}m{2cm}}
\newcolumntype{C}{>{\raggedright\arraybackslash}m{8.5cm}}
{\renewcommand{\arraystretch}{2}%

\clearpage
\onecolumn

\section{Authors' Response}

We are grateful to the reviewers for their helpful feedback and the opportunity to revise our submission. We used the additional two pages to expand our discussion of the issues they raised---especially why fitting models to both assign pre-defined classes and discover topics was useful, how the models should be used by political attention researchers, and how our approach differs from earlier work on Twitter and political communication. We summarize the reviewers' comments and point to our revisions in the table below. The reviewers' original comments are provided at the end. Thank you again for your time and help!

\section{Summary of Revisions}

\begin{supertabular}[ht!]

\begin{supertabular}{ABC}
\toprule
Comment & Reviewer 
% & Edit Plan 
& Revisions Made \\ \hline
\midrule
- Lack of technical novelty 
\linebreak
- value of the submission is in comparing the outputs and performance of relatively ``off-the-shelf" models for less-technical researchers who tend to rely on human annotation to show the potential of these (semi)automated approaches
& SPC, R1, R2 
%& Explain that technical novelty is not the main goal - a useable model is; include MPSA models to show simple model did better
& Our models' contributions lie primarily in their applications. We demonstrate that existing codebooks can be modeled effectively and thereby facilitate both longitudinal and comparative studies. We have revised the introduction, especially, to highlight these contributions. We also expanded the section on recommended uses for each model (p. 9). \\ \hline
- Better performing models elsewhere 
\linebreak 
- There are better performing state of the art techniques for analyzing tweets that would have affected the results.
& SPC, R1, R2 
%& I'm not sure what better performing models they are talking about, and R2 doesn't give any references. Quick lit search to see? 
& We have added additional details about different algorithms, document types, coherence measures we tested. These revisions can be found primarily on pp. 4-5. We also address some other techniques such as supervised LDA and network features in the future work section on p. 9-10.\\ \hline
criticizing employing a taxonomy of topics as a prior for fitting topics & SPC, R3 
% & Emphasize supervised for comparative work and unsupervised for the rest, connect to the sections about how to use these nearly-off-the-shelf tools 
& We acknowledge the tension between fitting topics to existing taxonomies and discovering new topic sets more explicitly (see p. 1). The CAP Codebook is so widely used in political communication research as a comparative tool that there is analytic utility in producing a supervised model that employs that taxonomy. We explain the importance and history of the CAP Codebook in additional references and discussion on p. 3 and expand on the discussion of when to use a supervised approach and when to use an unsupervised method on pp. 9-10.\\ \hline
The paper fails to establish that the problem, the use of the CAP codebook, is of any substantial prevalence in political communication research & R3 
% & Add a couple lines about the importance of CAP codebook in political science (with a bunch of references) 
& The Policy Agendas Project and the CAP codebook are widely-used in political science. We added citations to original Policy Agendas Project book \citep{Baumgartner1993-qq} and recent special issue and edited volume of examples \citep{Baumgartner2019-sx,John2006-rx} when the codebook is introduced (p. 3). Both Quinn et al. \citeyearpar{Quinn2010-nt} and Barber\'a et al. \citeyearpar{Barbera2018-bb,Barbera2014-pa} also map their codes to CAP. Given the space constraints, we aren't able to cite all the work that uses the CAP codebook and so instead cite a couple of especially significant studies and a recent edited volume. \\ \hline
- Distinguish from Quinn et al.
\linebreak
- clarify where its contribution lies in relation to (uncited) prior work also using or comparing semi-automated methods
\linebreak
- no evaluation comparison with other ML-based approaches
& SPC, R1, R3 
% & Add sentence or two around Quinn reference about the differences; Quinn didn't actually provide code for the model - the web site linked in the paper hasn't been updated since Jan 12, 2010 when it promises code in the next few days 
& Added paragraph in introduction that addresses Quinn et al. \citeyearpar{Quinn2010-nt} and Barber\'a et al. \citeyearpar{Barbera2018-bb,Barbera2014-pa} (pp. 1-2). We expanded the sections describing the specification and evaluation of our supervised model to include the other model specifications we tested (other algorithms and feature combinations) - see p. 3. \\ \hline
Labeling isn't that much work & R3 
% & Refs from political science about labeling, especially if crowdsourced labels were bad; Quinn on needing ``substantive knowledge" to label appropriately 
& Added reference to research about crowd sourcing for labeling political texts in introduction (Benoit etal., 2016; Haselmayer and Jenny, 2017; Lehmann and Zo-bel, 2018) on p. 1 \\ \hline
Is this about political attention & R3 
%& Maybe something like our MPSA introduction? 
& Added references to Twitter and political attention research to beginning of introduction \\ \hline
Enumerated items from R3 and copy-editing & R3 
%& See list and send to copy editor 
&
- Fixed typos and copy edits
\linebreak
- Addressed crowd sourcing and data labeling in introduction 
\linebreak
- Improved clarity in introduction about contributions and comparison to other approaches
\linebreak
- moved tables and figures to appear closer to their references
\\ \hline
\bottomrule
\end{supertabular}
\end{supertabluar}\mbox{}

\clearpage
\begin{enumerate}
\item Perhaps too nit-picky but I find the phrase "political attention" in the title
    is a bit misleading given that you are actually studying tweets posted by
    politicians, not really their attention to issue or the attentions of
    constituents/followers.
\item "Labeling content by hand requires tremendous human effort" -- we're talking
    about labelling tweets from ~500 people here, right? Seems like something that one
    full-time person could handle easily, or better yet crowdsourcing could resolve to
    some extent, certainly not a tremendous effort.
\item "Quinn and colleagues … provide a topic-modeling approach to classifying speech
    in the Congressional Record that is similar to ours." -- okay, but how is this
    work any different (aside from the obvious Tweets vs congressional record
    difference)?
\item MC is used before being introduced. 
\item Unclear: "mechanisms for estimating attention and style would provider richer
    views of activity and enable new analyses".
\item "To address these methodological challenges" -- thus far you didn't lay out the
    methodological challenges, just mentioned what people have done in the past.
\item As a paper that combines existing methods to apply to a specific problem, I
    expect to have a clear understanding by the end of the abstract (or at least by
    the end of the intro) of the general approach for evaluating your new tool and
    what were the finding from applying it to data. Both of these are currently
    missing.
\item " politicians’ behavior on Twitter demands our attention." -- too strong? 
\item "Twitter’s ready availability"?
\item "to answer these social and political research questions" -- what are the
    questions?
\item " tools or models for performing these analysis are currently unavailable" --
    didn't the work of Quinn et al. 2010 do just that?
\item The first paragraph in the data section doesn't add any value in my opinion. 
\item The exclusion of retweets requires further explanation, why focus only on
    "original" tweets?
\item "Nave Bayes".
\item Supervised classifier: what was the dependent variable more specifically?
\item Model specification: what is the unit of analysis? A tweet? That is likely to
    bias the model towards MC's that tweet more frequently. Why is that reasonable?
    You may want to consider the approach used in Barbera et al's work, which used all
    tweets from a single day as one document.
\item If you simply switched to use Krippendorff alpha it would save you some
    explaining.
\item "does not include a codes"
\item First paragraph under "Applying Models to 115th Congress’ Tweets" adds very
    little information.
\item Discussion on page 4 is very shallow. 
\item Can you place Fig. 1 closer to its reference? It is three pages away now.
\item "for each of those tweets those that".
\item " begs the question" -- that question is answerable from your results, isn't
    it?
\item "That none of the CAP Codebook topics energy,"
\item " That somewhere between 20 and 40 percent of all tweets are labeled with
    these topics tells us …"
\end{enumerate}

\section{Original Reviews}

===================Reviews for your paper follow===================

----------------------------------------------------------------

SPC/Associate Editor review

  Meta-Review and Roadmap

    The paper compares the performance of two modeling approaches for understanding
    political text generated by Members of Congress on their Twitter accounts.

    The reviewers all note the lack of technical novelty in the submission and R1 and
    R2 both note that there are better-performing models. I believe the value of the
    submission is in comparing the outputs and performance of relatively "off-the-
    shelf" models for less-technical researchers who tend to rely on human annotation
    to show the potential of these (semi)automated approaches.

    R3 notes the work by Quinn, et al. (2010) and Barbera, et al. (2014) criticizing
    employing a taxonomy of topics as a prior for fitting topics. The submission needs
    to clarify where its contribution lies in relation to (uncited) prior work also
    using or comparing semi-automated methods, offering something like a tutorial for
    social scientists to utilize these methods and models, providing deeper
    theoretical grounding than prior work, or richer qualitative interpretation of the
    results than prior technical reports.

----------------------------------------------------------------

reviewer/PC member 1 review

  Overall evaluation

    -2 = reject

  Reviewer's Confidence

    3 = Fairly confident that I've adequately considered all aspects

  Reviewer's methodological expertise

    3 = Knowledgeable: Knowledgeable in this methodological approach

  Paper summary

    The paper proposes two computational models to estimation political attention and
    to distinguish political topics in the politicians' Twitter tweets. The supervised
    model classifies the tweets into pre-defined topics. The unsupervised model
    uncovers the topics using topic modeling.

  Reasons to accept

    + The study of political attention in social media is interesting
    + Evaluation uses real data

  Reasons to reject

    + Low technical novelty and contribution
    + Lack of evaluation comparison with related work

  Comments for authors

    The analysis of political attention in social media sounds interesting. However,
    the major concern is the lack of novelty and technical contribution in this paper.
    The supervised model proposed simply uses the NLTK implementations of Naive Bayes
    and Logistic Regression to perform a standard classification. The unsupervised
    model proposed simply uses two variations of LDA for topic modeling. Thus, it
    sounds more like the paper applies some existing implementations to solve a
    problem, rather than proposing novelty techniques. Besides, there is no evaluation
    comparison with other Ml-based approaches. For example, SVM and random forest have
    demonstrated wide applicability in many areas, and thus it would be helpful to see
    how these approaches compare with the Naive Bayes and Logistic Regression
    implementations in this specific problem context.

  Originality of work

    Lack of novelty

  Potential impact of results

    Limited

  Quality of execution

    Needs improvement

  Quality of presentation

    Good

  Adequancy of citations

    Should include the citations of ML-based approaches and discuss their
    applicability

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------

reviewer/PC member 2 review

  Overall evaluation

    0 = borderline

  Reviewer's Confidence

    3 = Fairly confident that I've adequately considered all aspects

  Reviewer's methodological expertise

    3 = Knowledgeable: Knowledgeable in this methodological approach

  Paper summary

    The authors attempt to replace expensive manual labeling of politicians tweets
    that currently use established codebooks through computational means. The authors
    claim it would help in measuring political attention. They collect relevant data.
    They build a supervised classifier and a unsupervised topic model, and with the
    help of experts discuss their results. They find that topics that Republicans and
    Democrats give more attention to are mirrored in social media

  Reasons to accept

    The data collected is substantial and relevant to the problem, i.e., more than a
    million tweets of the members of the 115th Congress.

    The discussion of the labels generated by the unsupervised topic modeling and
    supervised classifier enable us to understand that this data can be used for other
    NLP/Text mining tasks such as single label to multi-label as well

  Reasons to reject

    There are better performing state of the art techniques for analyzing tweets that
    would have affected the results.

  Comments for authors

    Discussion on stemming for tweets may not be required. 
    some spellings need correction
    Unclear how many topics the CAP codebook has.
    A discussion on how CAP codes were assigned to inductive labeling would be
    helpful.
    Since 20 to 40 percent of tweets are considered not policy related but person to
    person and constituent service, perhaps they merit some discussion as well?
    would prefer more explanation on why foreign trade and international affairs are
    rare?

  Originality of work

    (blank)

  Potential impact of results

    The results indicate some underlying text mining problems such as single label to
    multi label classification and rare classes.

    For example foreign trade and international affairs are considered rare classes. 
    The example sorghum tweet is an example of a single label assigned where in it can
    be assigned to multiple labels, similarly for the labels defense and veteran
    affairs

  Quality of execution

    (blank)

  Quality of presentation

    (blank)

  Adequancy of citations

    (blank)

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------

reviewer/PC member 3 review

  Overall evaluation

    -1 = weak reject

  Reviewer's Confidence

    3 = Fairly confident that I've adequately considered all aspects

  Reviewer's methodological expertise

    3 = Knowledgeable: Knowledgeable in this methodological approach

  Paper summary

    The paper applies two computational models, supervised and unsupervised, to allow
    automatic and low-cost inference of topics discussed in tweets posted by members
    of congress. It also discusses the tradeoffs of the two models.

  Reasons to accept

    - The problem is interesting and important.
    - The paper does good computational science, engages in-depth with the results of
    quantitative method in light of social theory.
    - The methods used are reasonable and well-understood.

  Reasons to reject

    - Methodology: The computational methodology is not particularly novel (as an
    application paper this is insufficient reason to reject, but does put more
    emphasis on the novelty in other areas).
    - Contribution: It is not clear what this paper adds on top of the work of Quinn
    et al. 2010 and Barbera et al. 2014 (citation below). The main points about the
    use of predetermined taxonomy were already criticized by both papers. Also, the
    methodology is almost identical to these papers and the datasets used are only
    slightly different. If the focus was more specifically about the 115th congress I
    would understand this, but as a paper that examines the implications of particular
    methods I'm not clear what exactly is new here.
    - Problem statement: The paper fails to establish that the problem, the use of the
    CAP codebook, is of any substantial prevalence in political communication
    research. A quick google scholar search suggests very little support for that
    coding scheme being widely used. I may be wrong on this assessment since my area
    of expertise is not in political communication, but as a paper that contrasts
    different methods in that area I expect, at the very least, that the authors
    properly establish the prevalence of the problem. The existing support relies on
    two works from a single author (Russell).

    Barberá, Pablo, Richard Bonneau, Patrick Egan, John T. Jost, Jonathan Nagler, and
    Joshua Tucker. "Leaders or followers? Measuring political responsiveness in the US
    Congress using social media data." In 110th American Political Science Association
    Annual Meeting. 2014.

  Comments for authors

    My evaluation of this paper is based on (1) novelty of the approach being used,
    (2) quality of the evaluation, and (3) the overall quality of the presentation. I
    found the overall problem tackled in this paper interesting, the general approach
    reasonable, and the qualitative evaluation of the results rigorous and
    informative. However, due to the major issues I listed under 'reasons to reject'
    my recommendation is that the paper would not be accepted at this point. I
    encourage the authors to continue pursuing a publication on this work. In
    particular, I recommend that the authors flash out the contributions better and
    contrast them more directly with the work of Quinn et al. and Barbera et al.
    mentioned above. In addition, I would recommend that the main findings be stated
    earlier and more clearly.

    Other more minor issues/comments I noticed while reading the paper:
    1. Perhaps too nit-picky but I find the phrase "political attention" in the title
    is a bit misleading given that you are actually studying tweets posted by
    politicians, not really their attention to issue or the attentions of
    constituents/followers.
    2. "Labeling content by hand requires tremendous human effort" -- we're talking
    about labelling tweets from ~500 people here, right? Seems like something that one
    full-time person could handle easily, or better yet crowdsourcing could resolve to
    some extent, certainly not a tremendous effort.
    3. "Quinn and colleagues … provide a topic-modeling approach to classifying speech
    in the Congressional Record that is similar to ours." -- okay, but how is this
    work any different (aside from the obvious Tweets vs congressional record
    difference)?
    4. MC is used before being introduced. 
    5. Unclear: "mechanisms for estimating attention and style would provider richer
    views of activity and enable new analyses".
    6. "To address these methodological challenges" -- thus far you didn't lay out the
    methodological challenges, just mentioned what people have done in the past.
    7. As a paper that combines existing methods to apply to a specific problem, I
    expect to have a clear understanding by the end of the abstract (or at least by
    the end of the intro) of the general approach for evaluating your new tool and
    what were the finding from applying it to data. Both of these are currently
    missing.
    8. " politicians’ behavior on Twitter demands our attention." -- too strong? 
    9. "Twitter’s ready availability"?
    10. "to answer these social and political research questions" -- what are the
    questions?
    11. " tools or models for performing these analysis are currently unavailable" --
    didn't the work of Quinn et al. 2010 do just that?
    12. The first paragraph in the data section doesn't add any value in my opinion. 
    13. The exclusion of retweets requires further explanation, why focus only on
    "original" tweets?
    14. "Nave Bayes".
    15. Supervised classifier: what was the dependent variable more specifically?
    16. Model specification: what is the unit of analysis? A tweet? That is likely to
    bias the model towards MC's that tweet more frequently. Why is that reasonable?
    You may want to consider the approach used in Barbera et al's work, which used all
    tweets from a single day as one document.
    17. If you simply switched to use Krippendorff alpha it would save you some
    explaining.
    18. "does not include a codes"
    19. First paragraph under "Applying Models to 115th Congress’ Tweets" adds very
    little information.
    20. Discussion on page 4 is very shallow. 
    21. Can you place Fig. 1 closer to its reference? It is three pages away now.
    22. "for each of those tweets those that".
    23. " begs the question" -- that question is answerable from your results, isn't
    it?
    24. "That none of the CAP Codebook topics energy,"
    25. " That somewhere between 20 and 40 percent of all tweets are labeled with
    these topics tells us …"

  Originality of work

    The application of these (preexisting) methods to tweets from members of the 115th
    congress is new as well as the direct comparison with the result from learning a
    taxonomy. However, I am not exactly sure what this work adds beyond the work of
    Quinn et al and Barbera et al.

  Potential impact of results

    The results could inform analysis of political content in both the ICWSM community
    and in political communication.

  Quality of execution

    Very good. I appreciated especially the thorough qualitative assessment of the
    topics identified by LDA.

  Quality of presentation

    The paper needs a good copy editing, but otherwise mostly easy to read and follow.
    Nonetheless, it does need better focus on the main contributions, findings, and
    takeaways.

  Adequancy of citations

    Good, though I would recommend citing Barbera et al.'s work as it highly relevant
    to the current one.

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------
